Learn to Unlearn: A Survey on Machine Unlearning

Machine Learning (ML) models have been shown to potentially leak sensitive information, thus raising privacy concerns in ML-driven applications. This inspired recent research on removing the influence of specific data samples from a trained ML model. Such efficient removal would enable ML to comply with the "right to be forgotten" in many legislation, and could also address performance bottlenecks from low-quality or poisonous samples. In that context, machine unlearning methods have been proposed to erase the contributions of designated data samples on models, as an alternative to the often impracticable approach of retraining models from scratch. This article presents a comprehensive review of recent machine unlearning techniques, verification mechanisms, and potential attacks. We further highlight emerging challenges and prospective research directions (e.g. resilience and fairness concerns). We aim for this paper to provide valuable resources for integrating privacy, equity, andresilience into ML systems and help them "learn to unlearn".

==> table1.tex <==
{\color{blue}
\begin{longtable}{ p{1.4cm} p{1.5cm} p{1.5cm} p{2.1cm}p{5.5cm}p{4cm}}
    %\rowcolors{1}{gray!20}{white}
    \caption{\normalsize{Taxonomy of Machine Unlearning}}\\
    \label{table:accuracy} \\
    \hline
    \rowcolor{gray!60}
    \textbf{Category} & \textbf{Ref.} & \textbf{Dataset} & \textbf{Use Case} & \textbf{Main Contributions} & \textbf{Limitations}   \\
    \endfirsthead
    \rowcolor{gray!60}
    \textbf{Category} & \textbf{Ref.} & \textbf{Dataset} & \textbf{Use Case} & \textbf{Main Contributions} & \textbf{Limitations}   \\
    \endhead
    \hline
    \rowcolor{gray!20} Exact Unlearning   & Cao \textit{et al.}~\cite{cao2015towards} & Collected from Facebook & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Converting learning algorithms into a summation form for efficiently forgetting data lineage \end{tabular}} & {\begin{tabular}[p{5.5cm}]{@{}p{5.5cm}@{}}$\bullet$ The idea of forgetting systems that can restore privacy, security, and usability by completely and quickly erasing data lineage \\ $\bullet$ A universal unlearning method that transforms learning algorithms into a summation form, facilitating efficient forgetting of data lineage \\ $\bullet$ Real-world data pollution attacks developed against systems and algorithms \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Not every ML algorithm can be converted to the summation form \\ $\circ$ Data lineage at many levels of granularity is not considered \end{tabular}} \\
    \whiteline
                \rowcolor{gray!20} & Bourtoule \textit{et al.}~\cite{bourtoule2021machine} & Purchase, SVHN  & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}SISA: Data shard and incremental unlearning\end{tabular}} & {\begin{tabular}[p{5.5cm}]{@{}p{5.5cm}@{}} $\bullet$ Consider non-uniform distributions of unlearning requests \\ $\bullet$ Introduce SISA, which stands for Sharded, Isolated, Sliced, and Aggregated training \\ $\bullet$ Demonstrate that for complex learning tasks, a combination of transfer learning and SISA training results in a slight decrease in accuracy (\~ 2 percentage points) with improved retraining time. \end{tabular}} &  {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Performance degradation in each constituent model when datasets are too small, or if the learning task is complex \\ $\circ$ The unlearning through SISA is hard to verify \end{tabular}}  \\ 
    \whiteline
                \rowcolor{gray!20} & Wu \textit{et al.}~\cite{wu2020deltagrad} & MNIST, RCV1, HIGGS  & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Storing the original gradients, retaining the deleted data, and then integrating\end{tabular}} & {\begin{tabular}[p{5.5cm}]{@{}p{5.5cm}@{}} $\bullet$ Designed to quickly retrain ML models based on stochastic gradient descent, in response to small changes in the data, such as the addition or deletion of a small number of points \\ $\bullet$ Supported by theoretical results that demonstrate its accuracy, with the error being smaller than the fraction of points removed, for both GD and SGD methods \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Extra storage resources required to store the history gradients \\ $\circ$ Smaller mini-batch sizes in SGD is not supported \\ $\circ$ ML models without strong convexity may fail to converge \end{tabular}} \\ 
    \whiteline
                \rowcolor{gray!20} & Brophy \textit{et~al.}~\cite{brophy2021machine} & Adult, HIGGS, Bank, etc. & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Machine unlearning for random forests\end{tabular}} & {\begin{tabular}[p{5.5cm}]{@{}p{5.5cm}@{}} $\bullet$ Present a novel variant of random forests called DaRE, which enables the swift removal of training instances \\ $\bullet$ Assess DaRE's performance in handling sequences of deletions on 13 binary classification datasets from the real world \\ $\bullet$ Demonstrate that DaRE can remove data instances with a speed advantage of 2-4 orders, while incurring a predictive performance loss of less than 1\% \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ May leak privacy before and after deletion \\ $\circ$ Only applies to Random Forests \\ $\circ$ Lead to a slight degradation of predictive performance \end{tabular}}  \\
                
                
    \hline            
    \rowcolor{gray!30} Approx. Unlearning   & Guo \textit{et al.}~\cite{guo2020certified} & MNIST  & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Training a certified ML model considering the data removal in advance\end{tabular}} & {\begin{tabular}[p{5.5cm}]{@{}p{5.5cm}@{}} $\bullet$ Present a method for removing data points from $L_2$-regularized linear models, which are trained using a differentiable convex loss function, in a certified manner \\ $\bullet$ Utilize a Newton step to effectively remove the influence of the removed data point on the model parameters \\ $\bullet$ Proposes a technique for masking the residual by randomly perturbing the training loss to prevent adversaries from extracting information from the small residual \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Inverting the Hessian matrix required by the Newton update removal mechanism poses difficulties. \\ $\circ$ Not applicable to models with non-convex losses \\ $\circ$ A significant disparity exists between our data-dependent bound and the actual gradient residual norm \end{tabular}} \\
    \whiteline
                \rowcolor{gray!30} & Golatkar \textit{et al.}~\cite{golatkar2020eternal} & MNIST, CIFAR-10, Lacuna-10 & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Defining a forgetting Lagrangian to achieve selective forgetting for deep neural networks\end{tabular}} & {\begin{tabular}[p{5.5cm}]{@{}p{5.5cm}@{}} $\bullet$ Define ``selective forgetting'' for neural network unlearning models \\ $\bullet$ Proposea a scrubbing procedure that removes information from the trained weights without accessing the raw training data or re-training from sketch \\ $\bullet$ Derive a computable upper bound to the amount of the retained information that is efficient to compute even for DNNs. \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ It has been observed that if the pretraining assumption is not considered while forgetting, even minor perturbations during the initial critical learning phase can result in significant variations in the final solution \end{tabular}}\\
    \whiteline
                \rowcolor{gray!30} & Sekhari \textit{et al.}~\cite{sekhari2021remember} & No experimental evaluation & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Rigorous study of generalization in machine unlearning, where the goal is to perform well on previously unseen data points\end{tabular}} & {\begin{tabular}[p{5.5cm}]{@{}p{5.5cm}@{}} $\bullet$ Explore the number of samples that can be unlearned while preserving performance \\ $\bullet$ Do not rely on the availability of training data during sample deletion, distinguishing it from prior work \\ $\bullet$ Show a strict separation between DP and machine unlearning \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Fail to provide dimension dependent information-theoretic lower bound on the deletion capacity \\ $\circ$ Cannot deal with non-convex loss functions \end{tabular}} \\ 
    % \whiteline
    %             \rowcolor{gray!30} & Ginart \textit{et al.}~\cite{ginart2019making} & MNIST, CellType, Botnet & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Machine unlearning for K-means\end{tabular}} & {\begin{tabular}[p{5cm}]{@{}p{5cm}@{}} $\bullet$ Introduced and Characterized the problem of efficient data deletion in machine learning \\ $\bullet$ Propose two different solutions for achieving deletion efficiency in k-means clustering, both of which offer theoretical guarantees and strong empirical performance \\ $\bullet$ synthesize 4 general engineering principles that can guide the design of deletion-efficient learning systems \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Only supports the deletion of a single data point at one time \\ $\circ$ Only applies to K-means \\ $\circ$ An assumption that there is only one model and one corresponding dataset \end{tabular}} \\
    % \whiteline
    %             \rowcolor{gray!30} & Nguyen \textit{et al.}~\cite{nguyen2020variational} & Airline, Moon, Fashion MNIST & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Machine unlearning for variational Bayesian machine learning\end{tabular}} & {\begin{tabular}[p{5cm}]{@{}p{5cm}@{}} $\bullet$ Extend machine unlearning to Variational Bayesian Unlearning \\ $\bullet$ Evaluate unlearning methods on Bayesian models, sparse Gaussian process, logistic regression  \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ New vulnerabilities of model fraud attacks \\ $\circ$ Only applies to the variational inference frameworks of Bayesian machine learning  
    %             \end{tabular}} \\
                
    % \whiteline                  
    % \rowcolor{gray!40} Verification \& Attacks   & Sommer \textit{et al.}~\cite{sommer2022athena} & MNIST, CIFAR-10, Fashion MNIST, etc. & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Probabilistic verification of machine unlearning\end{tabular}} &  {\begin{tabular}[p{5cm}]{@{}p{5cm}@{}} $\bullet$ Framework for machine unlearning verification \\ $\bullet$ Use data backdoors for verifying machine unlearning \\ $\bullet$ Assess the verification performance using multiple datasets \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Constraints on data samples \\ $\circ$ Conflicting backdoor patterns \\ $\circ$ Risk of backdoor injection \\ $\circ$ Potential vulnerability to backdoor attack detection mechanisms  \end{tabular}}     \\
    % \whiteline
    %             \rowcolor{gray!40} & Chen \textit{et al.}~\cite{chen2021machine} & MNIST, CIFAR-10, Adult, etc. & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Proposed member inference attacks on machine unlearning\end{tabular}} &  {\begin{tabular}[p{5cm}]{@{}p{5cm}@{}} $\bullet$ Introduce a novel membership inference attack in the machine unlearning setting that aims to detect if a target sample is present in the training set of the original model \\ $\bullet$ Quantify the privacy risks in machine unlearning by examining membership inference attacks \\ $\bullet$ Devise 4 defense methods to avoid the privacy risks arising from this attack \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Performance drops for SISA method \\ $\circ$ Performance drops if the unlearned/updating samples represents more than 0.2\% \end{tabular}} \\
    % \whiteline
    %             \rowcolor{gray!40} & Marchant \textit{et al.}~\cite{marchant2022hard} & MNIST, Fashion-MNIST, etc. & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Poisoning attacks on certified machine unlearning\end{tabular}} & {\begin{tabular}[p{5cm}] {@{}p{5cm}@{}} $\bullet$ A novel poisoning attacks on machine unlearning \\ $\bullet$ Take into account different factors such as white-box and grey-box attacks, various perturbation geometries and bounds, balancing the attacker's objective optimality with the computation time, and the feasibility of long-term attack execution  \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Only targets on a particular category of machine unlearning models \\ $\circ$ May not work well if off-the-shell anomaly detection models have been deployed \end{tabular}} \\
    \hline
\end{longtable}
}

==> table2.tex <==
{\color{blue}
\begin{longtable}{ p{1.4cm} p{1.5cm} p{1.5cm} p{2.1cm}p{5.5cm}p{4cm}}
    %\rowcolors{1}{gray!20}{white}
    \caption{\normalsize{Taxonomy of Machine Unlearning}}\\
    % \label{table:accuracy} \\
    \hline
    \rowcolor{gray!60}
    \textbf{Category} & \textbf{Ref.} & \textbf{Dataset} & \textbf{Use Case} & \textbf{Main Contributions} & \textbf{Limitations}   \\
    \endfirsthead
    \rowcolor{gray!60}
    \textbf{Category} & \textbf{Ref.} & \textbf{Dataset} & \textbf{Use Case} & \textbf{Main Contributions} & \textbf{Limitations}   \\
    \endhead
    \hline
    % \rowcolor{gray!20} Exact Unlearning   & Cao \textit{et al.}~\cite{cao2015towards} & Collected from Facebook & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Converting learning algorithms into a summation form for efficiently forgetting data lineage \end{tabular}} & {\begin{tabular}[p{5cm}]{@{}p{5cm}@{}}$\bullet$ The idea of forgetting systems that can restore privacy, security, and usability by completely and quickly erasing data lineage \\ $\bullet$ A universal unlearning method that transforms learning algorithms into a summation form, facilitating efficient forgetting of data lineage \\ $\bullet$ Real-world data pollution attacks developed against systems and algorithms \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Not every ML algorithm can be converted to the summation form \\ $\circ$ Data lineage at many levels of granularity is not considered \end{tabular}} \\
    % \whiteline
    %             \rowcolor{gray!20} & Bourtoule \textit{et al.}~\cite{bourtoule2021machine} & Purchase, SVHN  & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}SISA: Data shard and incremental unlearning\end{tabular}} & {\begin{tabular}[p{5cm}]{@{}p{5cm}@{}} $\bullet$ Consider non-uniform distributions of unlearning requests \\ $\bullet$ Introduce SISA, which stands for Sharded, Isolated, Sliced, and Aggregated training \\ $\bullet$ Demonstrate that for complex learning tasks, a combination of transfer learning and SISA training results in a slight decrease in accuracy (\~ 2 percentage points) with improved retraining time. \end{tabular}} &  {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Performance degradation in each constituent model when datasets are too small, or if the learning task is complex \\ $\circ$ The unlearning through SISA is hard to verify \end{tabular}}  \\ 
    % \whiteline
    %             \rowcolor{gray!20} & Wu \textit{et al.}~\cite{wu2020deltagrad} & MNIST, RCV1, HIGGS  & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Storing the original gradients, retaining the deleted data, and then integrating\end{tabular}} & {\begin{tabular}[p{5cm}]{@{}p{5cm}@{}} $\bullet$ Designed to quickly retrain ML models based on stochastic gradient descent, in response to small changes in the data, such as the addition or deletion of a small number of points \\ $\bullet$ Supported by theoretical results that demonstrate its accuracy, with the error being smaller than the fraction of points removed, for both GD and SGD methods \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Extra storage resources required to store the history gradients \\ $\circ$ Smaller mini-batch sizes in SGD is not supported \\ $\circ$ ML models without strong convexity may fail to converge \end{tabular}} \\ 
    % \whiteline
    %             \rowcolor{gray!20} & Brophy \textit{et~al.}~\cite{brophy2021machine} & Adult, HIGGS, Bank, etc. & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Machine unlearning for random forests\end{tabular}} & {\begin{tabular}[p{5cm}]{@{}p{5cm}@{}} $\bullet$ Present a novel variant of random forests called DaRE, which enables the swift removal of training instances \\ $\bullet$ Assess DaRE's performance in handling sequences of deletions on 13 binary classification datasets from the real world \\ $\bullet$ Demonstrate that DaRE can remove data instances with a speed advantage of 2-4 orders, while incurring a predictive performance loss of less than 1\% \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ May leak privacy before and after deletion \\ $\circ$ Only applies to Random Forests \\ $\circ$ Lead to a slight degradation of predictive performance \end{tabular}}  \\
                
                
    % \whiteline            
    % \rowcolor{gray!30} Approx. Unlearning   & Guo \textit{et al.}~\cite{guo2020certified} & MNIST  & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Training a certified ML model considering the data removal in advance\end{tabular}} & {\begin{tabular}[p{5cm}]{@{}p{5cm}@{}} $\bullet$ Present a method for removing data points from $L_2$-regularized linear models, which are trained using a differentiable convex loss function, in a certified manner \\ $\bullet$ Utilize a Newton step to effectively remove the influence of the removed data point on the model parameters \\ $\bullet$ Proposes a technique for masking the residual by randomly perturbing the training loss to prevent adversaries from extracting information from the small residual \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Inverting the Hessian matrix required by the Newton update removal mechanism poses difficulties. \\ $\circ$ Not applicable to models with non-convex losses \\ $\circ$ A significant disparity exists between our data-dependent bound and the actual gradient residual norm \end{tabular}} \\
    % \whiteline
                % \rowcolor{gray!30} & Golatkar \textit{et al.}~\cite{golatkar2020eternal} & MNIST, CIFAR-10, Lacuna-10 & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Defining a forgetting Lagrangian to achieve selective forgetting for deep neural networks\end{tabular}} & {\begin{tabular}[p{5cm}]{@{}p{5cm}@{}} $\bullet$ Define ``selective forgetting'' for neural network unlearning models \\ $\bullet$ Proposea a scrubbing procedure that removes information from the trained weights without accessing the raw training data or re-training from sketch \\ $\bullet$ Derive a computable upper bound to the amount of the retained information that is efficient to compute even for DNNs. \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ It has been observed that if the pretraining assumption is not considered while forgetting, even minor perturbations during the initial critical learning phase can result in significant variations in the final solution \end{tabular}}\\
    % \whiteline
    %             \rowcolor{gray!30} & Sekhari \textit{et al.}~\cite{sekhari2021remember} & No experimental evaluation & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Rigorous study of generalization in machine unlearning, where the goal is to perform well on previously unseen data points\end{tabular}} & {\begin{tabular}[p{5.5cm}]{@{}p{5.5cm}@{}} $\bullet$ Explore the number of samples that can be unlearned while preserving performance \\ $\bullet$ Do not rely on the availability of training data during sample deletion, distinguishing it from prior work \\ $\bullet$ Show a strict separation between DP and machine unlearning \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Fail to provide dimension dependent information-theoretic lower bound on the deletion capacity \\ $\circ$ Cannot deal with non-convex loss functions \end{tabular}} \\ 
    \whiteline
                \rowcolor{gray!30} & Ginart \textit{et al.}~\cite{ginart2019making} & MNIST, CellType, Botnet & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Machine unlearning for K-means\end{tabular}} & {\begin{tabular}[p{5.5cm}]{@{}p{5.5cm}@{}} $\bullet$ Introduced and Characterized the problem of efficient data deletion in machine learning \\ $\bullet$ Propose two different solutions for achieving deletion efficiency in k-means clustering, both of which offer theoretical guarantees and strong empirical performance \\ $\bullet$ synthesize 4 general engineering principles that can guide the design of deletion-efficient learning systems \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Only supports the deletion of a single data point at one time \\ $\circ$ Only applies to K-means \\ $\circ$ An assumption that there is only one model and one corresponding dataset \end{tabular}} \\
    \whiteline
                \rowcolor{gray!30} & Nguyen \textit{et al.}~\cite{nguyen2020variational} & Airline, Moon, Fashion MNIST & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Machine unlearning for variational Bayesian machine learning\end{tabular}} & {\begin{tabular}[p{5.5cm}]{@{}p{5.5cm}@{}} $\bullet$ Extend machine unlearning to Variational Bayesian Unlearning \\ $\bullet$ Evaluate unlearning methods on Bayesian models, sparse Gaussian process, logistic regression  \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ New vulnerabilities of model fraud attacks \\ $\circ$ Only applies to the variational inference frameworks of Bayesian machine learning  
                \end{tabular}} \\
                
    \hline                 
    \rowcolor{gray!40} Verification \& Attacks   & Sommer \textit{et al.}~\cite{sommer2022athena} & MNIST, CIFAR-10, Fashion MNIST, etc. & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Probabilistic verification of machine unlearning\end{tabular}} &  {\begin{tabular}[p{5.5cm}]{@{}p{5.5cm}@{}} $\bullet$ Framework for machine unlearning verification \\ $\bullet$ Use data backdoors for verifying machine unlearning \\ $\bullet$ Assess the verification performance using multiple datasets \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Constraints on data samples \\ $\circ$ Conflicting backdoor patterns \\ $\circ$ Risk of backdoor injection \\ $\circ$ Potential vulnerability to backdoor attack detection mechanisms  \end{tabular}}     \\
    \whiteline
                \rowcolor{gray!40} & Chen \textit{et al.}~\cite{chen2021machine} & MNIST, CIFAR-10, Adult, etc. & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Proposed member inference attacks on machine unlearning\end{tabular}} &  {\begin{tabular}[p{5.5cm}]{@{}p{5.5cm}@{}} $\bullet$ Introduce a novel membership inference attack in the machine unlearning setting that aims to detect if a target sample is present in the training set of the original model \\ $\bullet$ Quantify the privacy risks in machine unlearning by examining membership inference attacks \\ $\bullet$ Devise 4 defense methods to avoid the privacy risks arising from this attack \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Performance drops for SISA method \\ $\circ$ Performance drops if the unlearned/updating samples represents more than 0.2\% \end{tabular}} \\
    \whiteline
                \rowcolor{gray!40} & Marchant \textit{et al.}~\cite{marchant2022hard} & MNIST, Fashion-MNIST, etc. & {\begin{tabular}[p{2.1cm}]{@{}p{2.1cm}@{}}Poisoning attacks on certified machine unlearning\end{tabular}} & {\begin{tabular}[p{5.5cm}] {@{}p{5.5cm}@{}} $\bullet$ A novel poisoning attacks on machine unlearning \\ $\bullet$ Take into account different factors such as white-box and grey-box attacks, various perturbation geometries and bounds, balancing the attacker's objective optimality with the computation time, and the feasibility of long-term attack execution  \end{tabular}} & {\begin{tabular}[p{4cm}]{@{}p{4cm}@{}} $\circ$ Only targets on a particular category of machine unlearning models \\ $\circ$ May not work well if off-the-shell anomaly detection models have been deployed \end{tabular}} \\
    \hline
\end{longtable}
}
